Mistral Supercomputer Job History Analysis

In this technical report, we show insights and results of operational data analysis from petascale supercomputer Mistral, which is ranked as 42nd most powerful in the world as of January 2018. Data sources include hardware monitoring data, job scheduler history, topology, and hardware information. We explore job state sequences, spatial distribution, and electric power patterns.

==> power_table_detailed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\centering
\caption{My caption}
\label{my-label}
\begin{adjustbox}{width=0.47\textwidth}

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Node profile} & \textbf{Jobs state} & \textbf{avg power {[}W{]}} & \textbf{avg/avg completed} \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_256 & COMPLETED           & 263                        & 1.00                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_256 & FAILED              & 238                        & 0.90                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_256 & CANCELLED           & 234                        & 0.89                       \\ \hline
B720-compute\_36\_128 & COMPLETED           & 247                        & 1.00                       \\ \hline
B720-compute\_36\_128 & FAILED              & 222                        & 0.90                       \\ \hline
B720-compute\_36\_128 & CANCELLED           & 231                        & 0.94                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_64  & COMPLETED           & 247                        & 1.00                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_64  & FAILED              & 223                        & 0.90                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_36\_64  & CANCELLED           & 226                        & 0.92                       \\ \hline
B720-compute\_24\_256 & COMPLETED           & 302                        & 1.00                       \\ \hline
B720-compute\_24\_256 & FAILED              & 275                        & 0.91                       \\ \hline
B720-compute\_24\_256 & CANCELLED           & 282                        & 0.93                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_24\_128 & COMPLETED           & 295                        & 1.00                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_24\_128 & FAILED              & 267                        & 0.90                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
B720-compute\_24\_128 & CANCELLED           & 276                        & 0.94                       \\ \hline
B720-compute\_24\_64  & COMPLETED           & 271                        & 1.00                       \\ \hline
B720-compute\_24\_64  & FAILED              & 255                        & 0.94                       \\ \hline
B720-compute\_24\_64  & CANCELLED           & 251                        & 0.92                       \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> table_sub_jobs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\setlength{\tabcolsep}{3pt}
\begin{table}[h]
\centering
\caption{Steps statistics by Slurm state}
\vspace{-5pt}
\label{table_job_steps}
\begin{adjustbox}{width=0.9\textwidth}

\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l}
\hline
\multirow{2}{*}{State} & \multirow{2}{*}{count} & \multicolumn{4}{l|}{\textbf{Allocated nodes}} & \multicolumn{4}{l|}{\textbf{Duration {[}s{]}}} & \multicolumn{4}{l|}{\textbf{Ave Disk Read {[}GB{]}}} & \multicolumn{4}{l}{\textbf{Ave Disk Write {[}GB{]}}} \\ \cline{3-18} 
                       &                        & mean      & SD      & min      & max      & mean      & SD      & min      & max       & mean        & SD        & min       & max        & mean        & SD        & min       & max         \\ \hline \hline
CANCELLED              & 53579                  & 28        & 87          & 1        & 3264     & 3322      & 8679        & 1        & 183k      & 16          & 151           & 0         & 7821       & 3           & 37            & 0         & 2341        \\ \hline
COMPLETED              & 4853842                & 3.4       & 17          & 1        & 3276     & 414       & 1902        & 1        & 235k      & 1           & 10            & 0         & 6993       & 0.2         & 5             & 0         & 30742       \\ \hline
FAILED                 & 197704                 & 18        & 28          & 1        & 3249     & 1111      & 5273        & 1        & 346k      & 3           & 73            & 0         & 6629       & 0.2         & 15            & 0         & 4078        \\ \hline
ALL                    & 5105125                & 4.2       & 20          & 1        & 3276     & 471       & 2326        & 1        & 346k      & 1           & 23            & 0         & 7821       & 0.2         & 7             & 0         & 4078        \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-20pt}
\end{table}
